Mitigating Boundary Ambiguity and Inherent Bias for Text Classification in the Era of Large Language Models

Text classification is a crucial task encountered frequently in practical scenarios, yet it is still under-explored in the era of large language models (LLMs). This study shows that LLMs are vulnerable to changes in the number and arrangement of options in text classification. Our extensive empirical analyses reveal that the key bottleneck arises from ambiguous decision boundaries and inherent biases towards specific tokens and positions. To mitigate these issues, we make the first attempt and propose a novel two-stage classification framework for LLMs. Our approach is grounded in the empirical observation that pairwise comparisons can effectively alleviate boundary ambiguity and inherent bias. Specifically, we begin with a self-reduction technique to efficiently narrow down numerous options, which contributes to reduced decision space and a faster comparison process. Subsequently, pairwise contrastive comparisons are employed in a chain-of-thought manner to draw out nuances and distinguish confusable options, thus refining the ambiguous decision boundary. Extensive experiments on four datasets (Banking77, HWU64, LIU54, and Clinic150) verify the effectiveness of our framework. Furthermore, benefitting from our framework, various LLMs can achieve consistent improvements. Our code and data are available in \url{https://github.com/Chuge0335/PC-CoT}.

==> algos/construct.tex <==
\begin{minipage}{\columnwidth}
    \begin{algorithm}[H]\small
    \caption{Demonstration-Construct}\label{alg:construct}
    \begin{algorithmic}[1]
    % \footnotesize
    \Require Sorted questions $\mathbf{q}^{(i)} = [q_1^{(i)}, q_2^{(i)}, \ldots]$ for each cluster $i$ ($i = 1, \ldots, k$), empty demonstration list $\mathbf{d}$
    \Ensure Demonstration list $\mathbf{d} = [d^{(1)}, \ldots, d^{(k)}]$ 
    \Procedure{Construct}{$\mathbf{q}^{(i)}, \ldots, \mathbf{q}^{(k)}$}
    \For{each cluster $i = 1, \ldots, k$}
    \For{each question $q_j^{(i)}$ in $\mathbf{q}^{(i)}$}
    \State Generate rationale $r_j^{(i)}$ and answer $a_j^{(i)}$ for $q_j^{(i)}$ using Zero-Shot-CoT
    \If{$q_j^{(i)}, r_j^{(i)}$ satisfy selection criteria}
        \State Add $d^{(i)} = [\text{Q: } q_j^{(i)}, \text{A: } r_j^{(i)} \circ a_j^{(i)}]$ to  $\mathbf{d}$
        \State \textbf{break}
    \EndIf
    \EndFor
    \EndFor
    \State \textbf{return} $\mathbf{d}$ 
    \EndProcedure%
    \end{algorithmic}
    \end{algorithm}
\end{minipage}

==> algos/reducer.tex <==
% \begin{minipage}{0.91\columnwidth}
% \begin{algorithm}[H]\small
% \caption{self-Reduction}\label{alg:cluster}
% \begin{algorithmic}[1]
% \Require A set of questions $\mathcal{Q}$ and the number of demonstrations $k$
% \Ensure Sorted questions $\mathbf{q}^{(i)} = [q_1^{(i)}, q_2^{(i)}, \ldots]$ for each cluster $i$ ($i = 1, \ldots, k$)
% \Procedure{Cluster}{$\mathcal{Q}$, $k$}
% \For{each question $q$ in $\mathcal{Q}$}
% \State Encode $q$ by Sentence-BERT
% \EndFor
% \State Cluster all the encoded question representations into $k$ clusters
% \For{each cluster $i = 1, \ldots, k$}
% \State Sort questions $\mathbf{q}^{(i)} = [q_1^{(i)}, q_2^{(i)}, \ldots]$ in the ascending order of the distance to the cluster center
% \EndFor
% \State \textbf{return} $\mathbf{q}^{(i)}$ ($i = 1, \ldots, k$)
% \EndProcedure%
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \hfill


% \begin{minipage}{0.91\columnwidth}
% \begin{algorithm}[H]\small
% \caption{Slide-Window}
% \begin{algorithmic}[1]
% \Require A textual sentence $\{x_i,y_i\}$ and the number of demonstrations $k$
% \Ensure Sorted questions $\mathbf{q}^{(i)} = [q_1^{(i)}, q_2^{(i)}, \ldots]$ for each cluster $i$ ($i = 1, \ldots, k$)
% \Procedure{Cluster}{$\mathcal{Q}$, $k$}
% \For{each question $q$ in $\mathcal{Q}$}
% \State Encode $q$ by Sentence-BERT
% \EndFor
% \State Cluster all the encoded question representations into $k$ clusters
% \For{each cluster $i = 1, \ldots, k$}
% \State Sort questions $\mathbf{q}^{(i)} = [q_1^{(i)}, q_2^{(i)}, \ldots]$ in the ascending order of the distance to the cluster center
% \EndFor
% \State \textbf{return} $\mathbf{q}^{(i)}$ ($i = 1, \ldots, k$)
% \EndProcedure%
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \hfill

% \begin{minipage}{0.91\columnwidth}
% \begin{algorithm}[H]\small
% \caption{Self-Reduction}
% \begin{algorithmic}[1]
% \Require A set of labels $\mathcal{Y}$, iteration number $T$ 
% \Ensure A reduced set of sorted labels $\mathbf{Y}_r = [y_1, y_2, \ldots, y_N]$
% \Procedure{Reduce}{$\mathcal{L}$}
% \While{for $t = 1, \cdots, T$}
% \State Select the most probable label $y_j$ from $\mathcal{Y}$ 
% \State Add $l$ to $\mathbf{l}$
% \State Remove $l$ from $\mathcal{L}$ to reduce the number of label options 
% \EndWhile
% \State \textbf{return} $\mathbf{l}$
% \EndProcedure%
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \hfill

% \begin{minipage}{0.91\columnwidth}
% \begin{algorithm}[H]\small
% \caption{Self-Reduction (TopK)}\label{alg:topk}
% \begin{algorithmic}[1]
% \Require Input sentence $x$, label options set $\mathcal{Y}= \{y_1,y_2,\cdots,y_N\}$, LLM $p_\theta$, evaluator $E()$, selection prompt \texttt{Sel}, step limit T.
% \State Initialize $S_0 = \mathcal{Y}$, $\mathcal{R}=\{\}$
% \For {$t = 1,\cdots,T$}
% \State $y_t \leftarrow \text{argmax}_y p_\theta^\texttt{Sel}(y | x,S_t) $
% \State $\mathcal{R} \leftarrow  \mathcal{R}\cup \{y_t\}$
% \State $S_{t+1} \leftarrow  \{ S_{t} \backslash \{y_t\} \}$
% \EndFor
% \State \textbf{return} $\mathcal{R}$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \hfill

==> algos/sampling.tex <==
\begin{minipage}{\columnwidth}
\begin{algorithm}[H]\small
\caption{Margin-Samping}\label{alg:cluster}
\begin{algorithmic}[1]
\Require A set of questions $\mathcal{Q}$ and the number of demonstrations $k$
\Ensure Sorted questions $\mathbf{q}^{(i)} = [q_1^{(i)}, q_2^{(i)}, \ldots]$ for each cluster $i$ ($i = 1, \ldots, k$)
\Procedure{Cluster}{$\mathcal{Q}$, $k$}
\For{each question $q$ in $\mathcal{Q}$}
\State Encode $q$ by Sentence-BERT
\EndFor
\State Cluster all the encoded question representations into $k$ clusters
\For{each cluster $i = 1, \ldots, k$}
\State Sort questions $\mathbf{q}^{(i)} = [q_1^{(i)}, q_2^{(i)}, \ldots]$ in the ascending order of the distance to the cluster center
\EndFor
\State \textbf{return} $\mathbf{q}^{(i)}$ ($i = 1, \ldots, k$)
\EndProcedure%
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill

==> figures/fewshot.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/fewshot.pdf}
    \caption{Accuracy for varying numbers of few shot demonstrations.}
    \label{fig:fs}
\end{figure}

==> figures/method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/arr2024_cot_p1.drawio.pdf}
    \caption{The reasoning process of our methods in classifying the two most probable classes.}
    \label{fig:main}
\end{figure*}

==> figures/options.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/option.pdf}
    \caption{Demonstration sampling methods comparison.}
    \label{fig:sec3-1}
\end{figure}


==> figures/silhouetted.tex <==
\begin{figure}[t]
    \centering
    \small
    \includegraphics[width=1\columnwidth]{figures/Silhouette.pdf}
    \caption{Demonstration sampling methods comparison.}
    \label{fig:sec3-3}
\end{figure}

==> figures/two-decision.tex <==

\begin{figure}[h]
    \centering
    \begin{subfigure}[h]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/Silhouette-0.pdf}
        \caption{ A higher silhouette score indicates clear boundaries between classes \label{fig:s0}}
    \end{subfigure}
    \begin{subfigure}[h]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/Silhouette-1.pdf}
        \caption{ A lower silhouette score suggesting overlapping classes. \label{fig:s1}}
    \end{subfigure}
    \caption{ Visualization of silhouette scores and decision boundaries }
    \label{fig:two}
\end{figure}


==> tables/benchmark.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{@{}lcccc@{}}
    \toprule
    Dataset & Classes & Sentences & Sent./Class & token/Sent.\\
    \midrule
    Banking & 77 & 13,083 & 170 & 12 \\
    HWU & 64 & 11,036 & 172 & 7 \\
    Clinic & 150 & 22,500 & 150 & 9 \\
    Liu & 54 & 25,478 & 472 & 8 \\
    \bottomrule
    \end{tabular}
    }
\caption{Your caption}
\label{tab:sec3-1}
\end{table}

==> tables/easy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\small
\centering
\resizebox{\linewidth}{!}{ 
\begin{tabular}{@{}cllllllll@{}}
    \toprule
    \multicolumn{1}{l}{Model} & Method & reminder & yahoo & agnews & bbcnews & mr & laptop & restaurant \\ 
    \midrule
    \multirow{3}{*}{ChatGPT3.5} & FS & 74.24 & \textbf{69.19} & 80.30 & 87.43 & \textbf{94.95} & 81.82 & 85.86 \\
     & FS-CoT & 78.79 & 65.66 & 81.31 & 92.19 & 93.94 & 83.33 & 86.98 \\
     & Mac-CoT & \textbf{79.69} & 65.15 & \textbf{82.83} & \textbf{92.25} & 90.91 & \textbf{84.80} & \textbf{87.37} \\
     \midrule
    \multirow{3}{*}{LLaMA-70B} & FS & 65.40 & 36.60 & 64.80 & 100.00 & 79.60 & 85.55 & 87.13 \\
     & FS-CoT & \textbf{75.10} & 42.10 & 63.00 & 100.00 & 77.00 & \textbf{85.78} & \textbf{87.95} \\
     & Mac-CoT & 74.90 & \textbf{57.60} & \textbf{82.20} & \textbf{100.00} & \textbf{87.30} & 83.89 & 87.29 \\
     \midrule
    \multirow{3}{*}{LLaMA-13B} & FS & 12.20 & 38.50 & 56.40 & 99.05 & 71.30 & 68.72 & \textbf{79.87} \\
     & FS-CoT & 13.60 & 41.00 & \textbf{63.70} & 99.05 & 75.50 & \textbf{78.67} & 77.06 \\
     & Mac-CoT & \textbf{38.90} & \textbf{39.60} & 61.60 & \textbf{99.05} & \textbf{78.20} & 76.54 & {74.36} \\ 
     \bottomrule
    \end{tabular}
    } 
\end{table*}

==> tables/inter_examples.tex <==

\begin{table*}[t]\centering
    \small
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{p{0.3\textwidth}|p{0.3\textwidth}|p{0.3\textwidth}}
    \toprule
    
    \textbf{Prompt} & \textbf{Chain of Thought} & \textbf{Margin-Chain of Thought}
    \\
    
    \midrule
\begin{tabular}{p{0.28\textwidth}}
\bblack{Q:} Below is a text classification problem, please complete the sentence by "get\_reminder" or "create\_reminder":  \\
\bblack{SENTENCE:} What are my reminders tonight? \\
\bblack{LABEL:} get\_reminder \\
\bblack{SENTENCE:} Set Reminder every August to schedule my yearly physical \\
\bblack{LABEL:} create\_reminder \\
\bblack{SENTENCE:} is there a reminder set to watch the news tomorrow if not set one? \\
\bblack{LABEL:} 
\end{tabular}
    &
\begin{tabular}{p{0.28\textwidth}}
\bblack{Q:} Below is a text classification problem. Let's think step by step and give your explanation to verify which term is more likely to represent the label of sentence - "get\_reminder" or "create\_reminder": \\
\bblack{SENTENCE:} What are my reminders tonight? \\
\bblack{EXPLANATION:} The label assigned to the sentence is "get\_reminder". This is because the sentence is a query asking about reminders, implying that the user is seeking information or assistance with reminders. \\
\bblack{LABEL:} get\_reminder \\
\bblack{SENTENCE:} Set Reminder every August to schedule my yearly physical \\
\bblack{EXPLANATION:} The statement mentions setting a reminder every August to schedule a yearly physical. This indicates an action related to creating a reminder, specifically for scheduling a regular health check-up. Therefore, the label assigned to this statement is "create\_reminder." \\
\bblack{LABEL:} create\_reminder \\
\bblack{SENTENCE:} is there a reminder set to watch the news tomorrow if not set one \\
\bblack{EXPLANATION:}
\end{tabular}
    &
\begin{tabular}{p{0.28\textwidth}}
\bblack{Q:} Below is a text classification problem: \\
\bblack{SENTENCE:} remind me about doctors appointment on monday \\
\bblack{LABEL:} create\_reminder \\
\bblack{SENTENCE:} Remind me about doctor's appointment on Tuesday not Monday. \\
\bblack{LABEL:} update\_reminder\_date\_time \\
\bblack{SIMILARITIES:} \\
- Both sentences involve a request to be reminded about a doctor's appointment. \\
% - Both sentences specify a specific day for the appointment (Monday in the first sentence and Tuesday in the second sentence). \\
\bblack{DIFFERENCES:} \\
- The first sentence simply asks for a reminder for a doctor's appointment on Monday. \\
- The second sentence updates the reminder, specifying that it should be for Tuesday instead of Monday. \\
\bblack{which term is more likely to represent the label of INPUT based on the SIMILARITIES and DIFFERENCES} - "create\_reminder" or "update\_reminder\_date\_time" : \\
\bblack{INPUT:} Update all reminders for the church group to 10 A.M. \\
\bblack{EXPLANATION:} \\
% - The sentence involves updating reminders for a specific group (the church group). \\
- The update specifically involves changing the time of the reminders to 10 A.M. \\
- This aligns with the context and actions typically associated with the "update\_reminder\_date\_time" label, which involves modifying existing reminders by changing the date and/or time. \\
\bblack{LABEL:} update\_reminder\_date\_time \\
\bblack{SENTENCE:} set a reminder for my doctor appointment \\
\bblack{LABEL:} create\_reminder \\
\bblack{SENTENCE:} Show my reminder for my doctor's appointment \\
\bblack{LABEL:} get\_reminder \\
\bblack{SIMILARITIES:}\\
- Both sentences involve a doctor appointment reminder. \\
% - The first sentence is a command to set a reminder for the appointment, while the second sentence is a command to display or retrieve the reminder. \\
\bblack{DIFFERENCES:} \\
- The first sentence is asking to set a reminder for a doctor appointment, indicating a request to create a new reminder. \\
- The second sentence is asking to show an existing reminder for a doctor's appointment, suggesting a request to retrieve an existing reminder.\\
\bblack{which term is more likely to represent the label of INPUT based on the SIMILARITIES and DIFFERENCES} - "create\_reminder" or "get\_reminder" : \\
\bblack{INPUT:} is there a reminder set to watch the news tomorrow if not set one \\
\bblack{EXPLANATION:}
\end{tabular}
    \\
\bottomrule
\end{tabular}
}
\caption{Examples of Retrieval-Q-CoT and Random-Q-CoT for constructing demonstrations and prediction. The upper part contains the automatically constructed demonstrations, and the lower part contains test questions along with predicted reasoning chains.}
\label{tab:pre_failure}
\end{table*}


    % \multirow{9}{0.3\textwidth}{
    % \bblack{A:} create\_reminder.\ngmark
    % &
    % \bblack{A:} The sentence is a query asking if there is a reminder set to watch the news tomorrow, and if not, it asks to set one. This implies that the user wants to check if there is a reminder and create one if necessary. Therefore, the label assigned to this sentence is "create\_reminder."LABEL: create\_reminder. \ngmark
    % &
    % \bblack{A:} Let's think step by step. The chef needs to cook 15 potatoes. He has already cooked 8. That means he has to cook 15-8=7 more potatoes. Each potato takes 9 minutes to cook. \textcolor{blue}{That means it will take him 9*7=63 minutes to cook \underline{\textbf{the rest}} of the potatoes.} The answer is 63. \okmark
    % \\
    % \bblack{Q:} A chef needs to cook 13 potatoes. He has already cooked 5. If each potato takes 6 minutes to cook, how long will it take him to cook \underline{\textbf{the rest}}?
    % &
    % \bblack{Q:} At a restaurant each adult meal costs \$5 and kids eat free. If a group of 15 people came in and 8 were kids, how much would it cost for the group to eat?
    % &
    % \bblack{Q:} A chef needs to cook 15 potatoes. He has already cooked 8. If each potato takes 9 minutes to cook, how long will it take him to cook \underline{\textbf{the rest}}?
    % \\
    % \bblack{A:} Let's think step by step. The chef has already cooked 5 potatoes. That means it has taken him 30 minutes so far. There are 13 potatoes in total. 5 have been cooked so far. That means there are 8 left to cook. Each potato takes 6 minutes to cook. That means it will take the chef 48 minutes to cook the 8 remaining potatoes. \textcolor{red}{In total, it will take the chef 78 minutes to cook all 13 potatoes.} The answer is 78.  \ngmark
    % &
    % \bblack{A:} Let's think step by step. There are 8 kids, so that means there are 7 adults. Each adult meal costs \$5, so that means that the 7 adults will cost \$5*7=\$35. Now we just need to add the two numbers together. \$35+8=43\$. So it would cost \$43 for the group to eat. The answer is 43.  \ngmark
    % &
    % \bblack{A:} Let's think step by step. The chef has already cooked 8 potatoes. That means it has taken him 8 * 9 minutes to cook those 8 potatoes. That means it will take him 9 minutes to cook each of the remaining 7 potatoes. \textcolor{red}{That means it will take him a total of 8 * 9 + 7 * 9 = 135 minutes to cook all 15 potatoes.} The answer is 135. \ngmark

==> tables/intra_examples.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{c|p{13.5cm} c}
            \bottomrule
            \multirow{3}{*}{{\textbf{Prompting Method}}}
            & \textbf{Classification Reasoning Example} \\ 
            & Question: Leah had 32 chocolates and her sister had 42. If they ate 35, how many pieces do they have left in total? \\
            \hline
            \multirow{1}{*}{{\textbf{Chain of Thought}}} 
            & Step-by-step answer: Originally, Leah had 32 chocolates and her sister had 42. So in total they had 32 + 42 = 74. After eating 35, they had 74 - 35 = 39 pieces left in total.The answer is 39. \\
            \hline
            \multirow{1}{*}{{\textbf{Failed: Similar linguistic}}} 
            & Step-by-step answer: Originally, Leah had 32 chocolates and her sister had 42. So in total they had 32 + 42 = 74. After eating 35, they had 74 - 35 = 39 pieces left in total.The answer is 39. \\
            \hline
            \multirow{1}{*}{{\textbf{Failed: Similar senmantic}}} 
            & Step-by-step answer: Originally, Leah had 32 chocolates and her sister had 42. So in total they had 32 + 42 = 74. After eating 35, they had 74 - 35 = 39 pieces left in total.The answer is 39. \\
            \hline
            \multirow{1}{*}{{\textbf{Failed: Similar intention}}} 
            & Step-by-step answer: Originally, Leah had 32 chocolates and her sister had 42. So in total they had 32 + 42 = 74. After eating 35, they had 74 - 35 = 39 pieces left in total.The answer is 39. \\
            \bottomrule
    \end{tabular}
    }
    \caption{Example cases. }
    \label{tab:case-2}
\end{table*}

==> tables/old.tex <==
\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Intent}} & \multicolumn{3}{c}{\textbf{Topic}} & \multicolumn{3}{c}{\textbf{Sentiment}}\\
\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} 
\multicolumn{1}{c}{} & \textbf{Reminder} & \textbf{AGNews} & \textbf{BBCNews} & \textbf{Yahoo} & \textbf{MR} & \textbf{Laptop} & \textbf{Restaurant} \\ \hline
Zero-Shot     & 90.20          & \textbf{81.86} & 92.45          & \textbf{60.66} & 84.00          & \textbf{82.70} & 85.81 \\
Zero-Shot-CoT & 90.60          & 79.38          & 91.77          & 59.16          & 82.60          & 81.99          & 86.47 \\
Few-Shot      & \textbf{97.50} & \textbf{87.60} & \textbf{94.50} & \textbf{61.20} & 90.86          & 79.62          & 86.96 \\
Few-Shot-CoT  & 96.60          & 84.30          & 92.70          & 60.30          & \textbf{91.40} & 81.75          & \textbf{87.46} \\
Mac-CoT       & \textbf{97.80} & 81.00          & \textbf{92.80} & 60.10          & \textbf{87.90} & 81.28          & \textbf{86.47} \\ \bottomrule
\end{tabular}
}
\caption{Differential ablation trials were conducted on various tasks using MAC-COT. Each architectural change resulted in significant performance gains, with the introduction of Different Prompt being particularly noteworthy.}
\label{tab0}
\end{table*}

==> tables/qwen.tex <==
% 5 shot
\begin{table*}[h]
\resizebox{\linewidth}{!}{ 
\begin{tabular}{llcccccccccccccccccccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{4}{c}{\textbf{Full Options}}  &  \multicolumn{5}{c}{\textbf{ Our Framework }} \\
 \cmidrule(r){3-6} \cmidrule(r){7-11} 
& & \textbf{ZS}    & \textbf{ZS-CoT}   & \textbf{FS}     & \textbf{FS-CoT}       & \textbf{ZS} & \textbf{ZS-CoT} & \textbf{FS} & \textbf{FS-CoT}& \textbf{PC-CoT}\\ \midrule
\multirow{5}{*}{\textbf{Qwen-1.8B-Chat}} 
& \textbf{Banking77}  & {18.18}  & {17.53}             & {4.87}   & {24.68}  & \underline{{26.62}}  & {23.7}      & {19.16}  & \textbf{{31.82}}      & {19.16} \\
& \textbf{HWU64 }   & {21.82}  & {22.73} & {4.55}  & {15.45}  & {24.55}  & \underline{{26.36}}      & {20.04}              & \textbf{{29.09}}         & {23.64} \\
& \textbf{LIU54}    & {17.32} & {17.32}  & {0.79}  & {18.11}    & \textbf{{23.62}}  & \underline{{20.47}}  & {17.72}      & {20.08}  & {17.32} \\
& \textbf{Clinc150} & {30.22}  & {33.78}             & {5.78}  & {20.89}  & \underline{{39.11}}  & {33.78}      & {35.56}              & \textbf{{54.22}}  & {25.78} \\
& \textbf{Average}  & {21.89}  & {22.84}              & {4.23}  & {19.78}  & \underline{{28.48}}  & {26.08}      & {23.11}  & \textbf{{33.80}}              & {21.48} \\ \midrule
\multirow{5}{*}{\textbf{Qwen-14B-Chat}} 
& \textbf{Banking77}  & {33.44}  & {33.12}             & {38.64}   & {46.43}  & {35.06}  & {26.62}      & \underline{{51.95}}  & {46.10}      & \textbf{{56.82}} \\
& \textbf{HWU64 }   & {40.01}  & {41.82} & {47.27}  & {50.02}  & {37.27}  & {38.18}      & \underline{{55.45}}              & {{53.64}}         & \textbf{{62.73}} \\
& \textbf{LIU54}    & {29.53} & {27.95}  & {31.50}  & {27.95}    & {31.10}  & {25.98}  & \underline{{37.40}}      & {32.28}  & \textbf{{38.19}} \\
& \textbf{Clinc150} & {53.78}  & {52.44}             & {58.22}  & {67.11}  & {{55.56}}  & {42.22}      & \underline{77.78}              & {{73.78}}  & \textbf{{82.67}} \\
& \textbf{Average}  & {39.19}  & {38.83}              & {43.91}  & {47.87}  & {39.75}  & {33.25}      & \underline{{55.65}}  & {51.45}              & {\textbf{60.35}} \\ \midrule
\multirow{5}{*}{\textbf{Qwen-72B-Chat}} 
& \textbf{Banking77}     & {43.83}  & {42.05}   & {48.70}  & {47.89}  & {49.68} & {44.97}  &           {53.09} & \underline{60.07}  & \textbf{61.69}\\
& \textbf{HWU64 }    & {54.55}  & {56.82}   & {55.00}  & {57.73}  & {43.64} & {47.73}  & \underline{60.46} &           {56.82}  & \textbf{63.64} \\
& \textbf{LIU54}     & {32.68}  & {31.10}   & {40.36}  & {36.62}  & {31.70} & {29.53}  & \underline{39.37} &           {38.78}  & \textbf{41.73} \\
& \textbf{Clinc150}  & {57.11}  & {58.00}   & {73.56}  & {73.56}  & {67.34} & {63.12}  &           {63.11} & \underline{83.78}  & \textbf{84.89} \\
& \textbf{Average}   & {47.04}  & {46.99}   & {54.40}  & {53.95}  & {48.09} & {46.34}  &           {54.01} & \underline{59.86}  & \textbf{62.99} \\ \bottomrule
\end{tabular}%
}
\caption{ Accuracy performance evaluation of encoder-only and decoder-only models. }
\label{tab:sft}
\vspace{-3mm}
\end{table*}

% \begin{table*}[t]
% \small
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{lccccccccccccccccccccccccccccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{4}{c}{\textbf{Full Options}}  &  \multicolumn{5}{c}{\textbf{ With Reducer }} \\
% \cmidrule(r){2-2} \cmidrule(r){3-6} \cmidrule(r){7-11} 
% & & \textbf{ZS}    & \textbf{ZS-CoT}   & \textbf{FS}     & \textbf{FS-CoT}       & \textbf{ZS} & \textbf{ZS-CoT} & \textbf{FS} & \textbf{FS-CoT}& \textbf{Mac-CoT}\\ \midrule
% \textbf{Banking}  & {33.44}  & {33.12}             & {38.64}   & {46.43}  & {35.06}  & {26.62}      & \underline{{51.95}}  & {46.10}      & \textbf{{56.82}} \\
% \textbf{HWU64 }   & {40}  & {41.82} & {47.27}  & {50}  & {37.27}  & {38.18}      & \underline{{55.45}}              & \textbf{{53.64}}         & \textbf{{62.73}} \\
% \textbf{LIU54}    & {29.53} & {27.95}  & {31.50}  & {27.95}    & {31.10}  & {25.98}  & \underline{{37.40}}      & {32.28}  & \textbf{{38.19}} \\
% \textbf{Clinc150} & {53.78}  & {52.44}             & {58.22}  & {67.11}  & \underline{{55.56}}  & {42.22}      & {77.78}              & \textbf{{73.78}}  & \textbf{{82.67}} \\
% \textbf{Average}  & {39.19}  & {38.83}              & {43.91}  & {47.87}  & {39.75}  & {33.25}      & \underline{{55.65}}  & {51.45}              & {\textbf{60.35}} \\ \bottomrule

% \end{tabular}%
% }
% \caption{ Qwen-chat(14B) 5-shot  }
% \label{tab:com}
% \end{table*}

% \begin{table*}[t]
% \small
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{lccccccccccccccccccccccccccccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{4}{c}{\textbf{Full Options}}  &  \multicolumn{5}{c}{\textbf{ With Reducer }} \\
% \cmidrule(r){2-2} \cmidrule(r){3-6} \cmidrule(r){7-11} 
% & & \textbf{ZS}    & \textbf{ZS-CoT}   & \textbf{FS}     & \textbf{FS-CoT}       & \textbf{ZS} & \textbf{ZS-CoT} & \textbf{FS} & \textbf{FS-CoT}& \textbf{Mac-CoT}\\ \midrule
% \textbf{Banking}  & {52}    & {42.53}  & {42.21}             & {50.97}   & {49.35}  & {49.35}  & {44.81}      & {49.68}  & \underline{{56.49}}      & \textbf{{62.34}} \\
% \textbf{HWU64 }   & {54}    & {56.36}  & {60} & {54.55}  & {57.27}  & {43.64}  & {47.27}      & \underline{{62.73}}              & \textbf{{57.27}}         & \textbf{{64.55}} \\
% \textbf{LIU54}    & {35}    & {28.74} & {29.92}  & {37.40}  & {37.01}    & \textbf{{31.89}}  & {29.53}  & {37.40}      & \underline{{38.58}}  & \textbf{{42.52}} \\
% \textbf{Clinc150} & {84}    & {57.78}  & {56.44}             & {75.11}  & {76.44}  & \underline{{67.11}}  & {63.56}      & {60.44}              & {84.00}  & \textbf{{84.89}} \\
% \textbf{Average}  & {56.25} & {46.35}  & {47.14}              & {54.51}  & {55.02}  & {48}  & {46.29}      & {52.56}  & \underline{{59.09}}              & {\textbf{63.58}} \\ \bottomrule

% \end{tabular}%
% }
% \caption{ Qwen-chat(72B) 5-shot  }
% \label{tab:com}
% \end{table*}

==> tables/sec3-1.tex <==
\begin{table}[ht]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{@{}lcccc@{}}
    \toprule
    Dataset & Classes & Sentences & Sent./Class & token/Sent.\\
    \midrule
    Banking & 77 & 13,083 & 170 & 12 \\
    HWU & 64 & 11,036 & 172 & 7 \\
    Clinic & 150 & 22,500 & 150 & 9 \\
    Liu & 54 & 25,478 & 472 & 8 \\
    \bottomrule
    \end{tabular}
    }
\caption{Your caption}
\label{tab:sec3-1}
\end{table}

==> tables/sec3-3.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{@{}lcc@{}}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{Sampling Methods}}& \multicolumn{2}{c}{Few-Shot} \\ 
    \cmidrule(lr){2-3}
    & K=1 & K=3 \\
    \midrule
    Center Sampling & 71 & 68 \\
    Random Sampling & 68 & 73 \\
    Contrastive Sampling & 67 & 74 \\
    \bottomrule
    \end{tabular}
    \caption{Your caption}
\label{tab:sec.3-3}
\end{table}

==> tables/sim_examples.tex <==

\begin{table*}[h]\centering
    \small
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{p{0.3\textwidth}|p{0.3\textwidth}|p{0.3\textwidth}}
    \toprule
    
    \textbf{Zero-Shot Reasoning} & \textbf{Zero-shot CoT Reasoning} & \textbf{Few-shot CoT Reasoning}
    \\
    
    \midrule
\begin{tabular}[t]{p{0.28\textwidth}}
\bblack{Q:} Given the sentence: "So I just put my top-up into the card and it hasn't changed." Please select the most possible topic from the following options.\\
\bblack{OPTIONS:} pending\_top\_up, top\_up\_failed, topping\_up\_by\_card, card\_not\_working, balance\_not\_updated, ...\\
\bblack{CHOICE:} \\
\\
\bblack{A:} The most possible topic for the given sentence is \textbf{topping\_up\_by\_card}. \ngmark
\\
\\
\hline
\vspace{0.2pt}
\textbf{Few-shot Reasoning} \\
\\
\bblack{Q:} Below is a text classification problem, Note that you can only select label in pending\_top\_up, top\_up\_failed, topping\_up\_by\_card, card\_not\_working, balance\_not\_updated, ... \\
\bblack{SENTENCE:} How long will it take for my cash withdrawal to no longer show as pending? \\
\bblack{LABEL:} pending\_cash\_withdrawal \\
... \\
\bblack{SENTENCE:} So I just put my top-up into the card and it hasn't changed. \\
\bblack{LABEL:} \\
\\
\bblack{A:} \textbf{card\_not\_working}\ngmark
\end{tabular}
    &
\begin{tabular}[t]{p{0.28\textwidth}}

\bblack{Q:} Given the sentence: "So I just put my top-up into the card and it hasn't changed." Please select the most possible topic from the following options.\\
\bblack{OPTIONS:} pending\_top\_up, top\_up\_failed, topping\_up\_by\_card, card\_not\_working, balance\_not\_updated, ...\\
Let's think step by step and verify your answer: \\
\\
\bblack{A:}Based on the given sentence "So I just put my top-up into the card and it hasn't changed," the most relevant topic seems to be \textbf{top\_up\_failed.} This is because the user mentions putting a top-up into the card, and there is an indication that something has not changed as expected. \ngmark\\
\end{tabular}
    &
\begin{tabular}[t]{p{0.28\textwidth}}
\bblack{Q:} Below is a text classification problem, Note that you can only select label in pending\_top\_up, top\_up\_failed, topping\_up\_by\_card, card\_not\_working, balance\_not\_updated, ... Let's think step by step and give your explanation to verify the answer. \\
\bblack{SENTENCE:} I topped up but it isn't in my account \\
\bblack{EXPLANATION:} The statement is about a user's concern regarding a top-up that has not been reflected in their account, which is related to a pending transaction or issue with their account balance. \\
\bblack{LABEL:} pending\_top\_up \\
... \\
\bblack{SENTENCE:} So I just put my top-up into the card and it hasn't changed. \\
\bblack{EXPLANATION:} \\
\\
\bblack{A:} The sentence is about a user who has topped up their card with money, but the balance has not been updated. This issue is related to the balance not being updated after a bank transfer, which falls under the label balance\_not\_updated\_after\_bank\_transfer. \\
LABEL: \textbf{balance\_not\_updated} \ngmark
\end{tabular}
 \\
\end{tabular}
}
\bottomrule
\label{tab:case}
\caption{Examples of Retrieval-Q-CoT and Random-Q-CoT for constructing demonstrations and prediction. The upper part contains the automatically constructed demonstrations, and the lower part contains test questions along with predicted reasoning chains.}
\end{table*}

==> tables/table0.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}cccccccccc@{}}
        \hline
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Intent}} & \multicolumn{3}{c}{\textbf{Topic}} & \multicolumn{3}{c}{\textbf{Sentiment}}\\
        \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} 
        \multicolumn{1}{c}{} & \textbf{Banking} & \textbf{Clinc} & \textbf{Reminder} & \textbf{AGNews} & \textbf{BBCNews} & \textbf{Yahoo} & \textbf{MR} & \textbf{Laptop} & \textbf{Restaurant} \\ \hline
        \textbf{Zero-shot} &  &  &  &  \\
        Prompt & 83.08 & 93.49  & 90.20 & \textbf{81.86} & 92.45 & \textbf{60.66} & 84.00 & \textbf{82.70} & 85.81 \\
        CoT & 81.64 & 90.80 & 90.60 & 79.38 & 91.77 & 59.16 & 82.60 & 81.99 & 86.47 \\
        Mac-CoT & \textbf{88.90} & \textbf{96.00} & \textbf{97.80} & 81.00 & \textbf{92.80} & 86.47 & \textbf{87.90} & 81.28 & \textbf{81.28} \\ \midrule
        \textbf{Few-shot} &  &  &  &  &  &  &     &  &  \\ 
    Prompt  &         &       & \textbf{97.50} & \textbf{87.60} & \textbf{94.50} & \textbf{61.20} & 90.86          & 79.62          & 86.96          \\
    CoT     &         &       & 96.60          & 84.30          & 92.70          & 60.30          & \textbf{91.40} & 81.75          & \textbf{87.46} \\
    Mac-CoT &         &       & 92.20          & 83.00          & 90.60          & 58.30          & 77.83          & \textbf{82.46} & 84.82          \\ \bottomrule
        \end{tabular}
        }
        \caption{Differential ablation trials were conducted on various tasks using MAC-COT. Each architectural change resulted in significant performance gains, with the introduction of Different Prompt being particularly noteworthy.}
        \label{tab:preliminary}
    \end{table*}

==> tables/table1.tex <==

\begin{table*}[t]
    \small
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{lllllll}
        \hline
        \textbf{Prompting Method} & \textbf{Clinc} & \textbf{Banking} & \textbf{Reminder} & \textbf{Restaurant} & \textbf{Avg.} \\
        \hline
        MacCOT & \textbf{96.00} & 88.90 & 97.80 & 86.47 & 92.29\\
        wo/ Differ Reasoning & 93.60 & 88.40 & 97.30 & 85.48 & 91.20\\
        wo/ Same Reasoning & 95.50 & 89.74 & \textbf{98.30} & \textbf{86.80} & 92.43\\
        wo/ Contrastive Reasoning & 95.80 & \textbf{90.29} & 98.30 & 85.62 & \textbf{92.50}\\
        \hline
            \end{tabular}}
        \caption{Differential ablation trials were conducted on various tasks using MAC-COT. Each architectural change resulted in significant performance gains, with the introduction of Different Prompt being particularly noteworthy.}
        \label{tab:preliminary}
    \end{table*}

==> tables/table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
    \begin{tabular}{lllllllll}
    \hline
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{Snips} & \multicolumn{4}{c}{Banking} \\ \cmidrule(r){2-5} \cmidrule(r){6-9} 
    \multicolumn{1}{c}{} & ACC & MaF1 & MiF1 & ARI & ACC & MaF1 & MiF1 & ARI \\ \hline
    CCoT(Random Sample) & 94.21 & 0.94 & 0.94 & 86.75 & 68.90 & 0.67 & 0.69 & 48.67 \\
    CCoT(Center Sample) & 93.21 & 0.93 & 0.93 & 84.85 & \textbf{69.97} & 0.68 & 0.70 & \textbf{49.80} \\
    CCoT(Boundary Sample) & \textbf{94.29} & \textbf{0.94} & \textbf{0.94} & \textbf{87.22} & 69.61 & \textbf{0.68} & \textbf{0.70} & 49.36 \\ \hline
    \end{tabular}
    \end{table*}
